Can We Trust Race Prediction?

In the absence of sensitive race and ethnicity data, researchers, regulators, and firms alike turn to proxies. In this paper, I train a Bidirectional Long Short-Term Memory (BiLSTM) model on a novel dataset of voter registration data from all 50 US states and create an ensemble that achieves up to 36.8% higher out of sample (OOS) F1 scores than the best performing machine learning models in the literature. Additionally, I construct the most comprehensive database of first and surname distributions in the US in order to improve the coverage and accuracy of Bayesian Improved Surname Geocoding (BISG) and Bayesian Improved Firstname Surname Geocoding (BIFSG). Finally, I provide the first high-quality benchmark dataset in order to fairly compare existing models and aid future model developers.

==> tables/bifsg_stats_max.tex <==
\begin{tabular}{lllllll}
\toprule
Race & Accuracy & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
Asian & 0.989 & 0.942 & 0.823 & 0.879 & 0.589 & 7,187 \\
Black & 0.941 & 0.7 & 0.616 & 0.656 & 0.536 & 13,957 \\
Hispanic & 0.949 & 0.928 & 0.797 & 0.858 & 0.764 & 29,881 \\
White & 0.904 & 0.902 & 0.961 & 0.931 & 0.843 & 103,437 \\
\bottomrule
\end{tabular}


==> tables/bifsg_stats_thresh50.tex <==
\begin{tabular}{lllllll}
\toprule
Race & Accuracy & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
Asian & 0.991 & 0.952 & 0.838 & 0.891 & 0.562 & 6,854 \\
Black & 0.944 & 0.711 & 0.622 & 0.664 & 0.52 & 13,542 \\
Hispanic & 0.951 & 0.932 & 0.804 & 0.863 & 0.753 & 29,421 \\
White & 0.908 & 0.906 & 0.963 & 0.934 & 0.838 & 102,779 \\
\bottomrule
\end{tabular}


==> tables/bisg_stats.tex <==
\begin{tabular}{lrrrrr}
\toprule
Race & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
asian & 0.864000 & 0.844000 & 0.854000 & 0.839000 & 12202 \\
black & 0.703000 & 0.654000 & 0.678000 & 0.900000 & 26059 \\
hispanic & 0.914000 & 0.806000 & 0.857000 & 0.919000 & 39089 \\
white & 0.874000 & 0.928000 & 0.900000 & 0.817000 & 122647 \\
\bottomrule
\end{tabular}


==> tables/bisg_stats_max.tex <==
\begin{tabular}{lllllll}
\toprule
Race & Accuracy & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
Asian & 0.986 & 0.904 & 0.842 & 0.872 & 0.875 & 10,674 \\
Black & 0.915 & 0.689 & 0.675 & 0.682 & 0.947 & 24,673 \\
Hispanic & 0.943 & 0.913 & 0.794 & 0.849 & 0.947 & 37,008 \\
White & 0.882 & 0.882 & 0.93 & 0.905 & 0.902 & 110,663 \\
\bottomrule
\end{tabular}


==> tables/bisg_stats_thresh50.tex <==
\begin{tabular}{lllllll}
\toprule
Race & Accuracy & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
Asian & 0.988 & 0.922 & 0.858 & 0.889 & 0.844 & 10,297 \\
Black & 0.922 & 0.703 & 0.688 & 0.695 & 0.892 & 23,239 \\
Hispanic & 0.946 & 0.919 & 0.806 & 0.859 & 0.926 & 36,214 \\
White & 0.89 & 0.889 & 0.936 & 0.912 & 0.887 & 108,805 \\
\bottomrule
\end{tabular}


==> tables/ensemble_stats.tex <==
\begin{tabular}{lrrrrr}
\toprule
Race & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
asian & 0.739000 & 0.860000 & 0.795000 & 1.000000 & 12202 \\
black & 0.710000 & 0.799000 & 0.752000 & 1.000000 & 26059 \\
hispanic & 0.883000 & 0.804000 & 0.842000 & 1.000000 & 39089 \\
white & 0.919000 & 0.906000 & 0.912000 & 1.000000 & 122647 \\
\bottomrule
\end{tabular}


==> tables/ensemble_stats_max.tex <==
\begin{tabular}{lllllll}
\toprule
Race & Accuracy & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
Asian & 0.979 & 0.803 & 0.862 & 0.831 & 1.0 & 12,202 \\
Black & 0.931 & 0.706 & 0.811 & 0.755 & 1.0 & 26,059 \\
Hispanic & 0.943 & 0.895 & 0.802 & 0.846 & 1.0 & 39,089 \\
White & 0.9 & 0.921 & 0.915 & 0.918 & 1.0 & 122,647 \\
\bottomrule
\end{tabular}


==> tables/ensemble_stats_thresh50.tex <==
\begin{tabular}{lllllll}
\toprule
Race & Accuracy & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
Asian & 0.981 & 0.828 & 0.871 & 0.849 & 0.974 & 11,883 \\
Black & 0.935 & 0.716 & 0.821 & 0.765 & 0.971 & 25,298 \\
Hispanic & 0.946 & 0.9 & 0.811 & 0.853 & 0.983 & 38,442 \\
White & 0.905 & 0.925 & 0.921 & 0.923 & 0.987 & 121,105 \\
\bottomrule
\end{tabular}


==> tables/eth_stats.tex <==
\begin{tabular}{lrrrrr}
\toprule
Race & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
asian & 0.870000 & 0.626000 & 0.728000 & 1.000000 & 12202 \\
black & 0.665000 & 0.461000 & 0.545000 & 1.000000 & 26059 \\
hispanic & 0.872000 & 0.756000 & 0.810000 & 1.000000 & 39089 \\
white & 0.827000 & 0.939000 & 0.879000 & 1.000000 & 122647 \\
\bottomrule
\end{tabular}


==> tables/eth_stats_thresh50.tex <==
\begin{tabular}{lllllll}
\toprule
Race & Accuracy & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
Asian & 0.977 & 0.918 & 0.667 & 0.773 & 0.919 & 11,214 \\
Black & 0.905 & 0.69 & 0.471 & 0.56 & 0.958 & 24,966 \\
Hispanic & 0.936 & 0.893 & 0.763 & 0.823 & 0.976 & 38,142 \\
White & 0.851 & 0.834 & 0.948 & 0.888 & 0.988 & 121,117 \\
\bottomrule
\end{tabular}


==> tables/fl_bayes_stats.tex <==
\begin{tabular}{lrrrrr}
\toprule
Race & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
asian & 0.677000 & 0.862000 & 0.759000 & 0.993000 & 12202 \\
black & 0.671000 & 0.842000 & 0.747000 & 1.000000 & 26059 \\
hispanic & 0.870000 & 0.808000 & 0.838000 & 0.999000 & 39089 \\
white & 0.933000 & 0.878000 & 0.905000 & 1.000000 & 122647 \\
\bottomrule
\end{tabular}


==> tables/fl_bayes_stats_max.tex <==
\begin{tabular}{lllllll}
\toprule
Race & Accuracy & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
Asian & 0.974 & 0.744 & 0.864 & 0.799 & 0.994 & 12,130 \\
Black & 0.925 & 0.664 & 0.854 & 0.747 & 1.0 & 26,046 \\
Hispanic & 0.941 & 0.881 & 0.805 & 0.841 & 0.999 & 39,052 \\
White & 0.893 & 0.934 & 0.888 & 0.911 & 1.0 & 122,601 \\
\bottomrule
\end{tabular}


==> tables/fl_bayes_stats_thresh50.tex <==
\begin{tabular}{lllllll}
\toprule
Race & Accuracy & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
Asian & 0.976 & 0.766 & 0.871 & 0.816 & 0.979 & 11,947 \\
Black & 0.928 & 0.674 & 0.861 & 0.756 & 0.979 & 25,524 \\
Hispanic & 0.943 & 0.887 & 0.813 & 0.848 & 0.985 & 38,504 \\
White & 0.898 & 0.937 & 0.894 & 0.915 & 0.985 & 120,798 \\
\bottomrule
\end{tabular}


==> tables/fl_stats.tex <==
\begin{tabular}{lrrrrr}
\toprule
Race & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
asian & 0.686000 & 0.833000 & 0.753000 & 1.000000 & 12202 \\
black & 0.577000 & 0.690000 & 0.628000 & 1.000000 & 26059 \\
hispanic & 0.851000 & 0.797000 & 0.823000 & 1.000000 & 39089 \\
white & 0.893000 & 0.855000 & 0.873000 & 1.000000 & 122647 \\
\bottomrule
\end{tabular}


==> tables/fl_stats_max.tex <==
\begin{tabular}{lllllll}
\toprule
Race & Accuracy & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
Asian & 0.975 & 0.772 & 0.839 & 0.804 & 1.0 & 12,202 \\
Black & 0.898 & 0.589 & 0.705 & 0.642 & 1.0 & 26,059 \\
Hispanic & 0.937 & 0.871 & 0.795 & 0.831 & 1.0 & 39,089 \\
White & 0.862 & 0.896 & 0.876 & 0.886 & 1.0 & 122,647 \\
\bottomrule
\end{tabular}


==> tables/fl_stats_thresh50.tex <==
\begin{tabular}{lllllll}
\toprule
Race & Accuracy & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
Asian & 0.977 & 0.788 & 0.851 & 0.818 & 0.977 & 11,925 \\
Black & 0.903 & 0.606 & 0.713 & 0.655 & 0.969 & 25,248 \\
Hispanic & 0.939 & 0.876 & 0.804 & 0.838 & 0.985 & 38,506 \\
White & 0.869 & 0.901 & 0.884 & 0.892 & 0.978 & 119,997 \\
\bottomrule
\end{tabular}


==> tables/ibifsg_stats.tex <==
\begin{tabular}{lrrrrr}
\toprule
Race & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
asian & 0.876000 & 0.876000 & 0.876000 & 0.732000 & 12202 \\
black & 0.730000 & 0.759000 & 0.744000 & 0.748000 & 26059 \\
hispanic & 0.912000 & 0.824000 & 0.866000 & 0.853000 & 39089 \\
white & 0.914000 & 0.936000 & 0.925000 & 0.804000 & 122647 \\
\bottomrule
\end{tabular}


==> tables/ibifsg_stats_max.tex <==
\begin{tabular}{lllllll}
\toprule
Race & Accuracy & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
Asian & 0.988 & 0.905 & 0.873 & 0.889 & 0.764 & 9,325 \\
Black & 0.936 & 0.713 & 0.766 & 0.738 & 0.786 & 20,487 \\
Hispanic & 0.947 & 0.911 & 0.813 & 0.859 & 0.881 & 34,433 \\
White & 0.908 & 0.917 & 0.939 & 0.928 & 0.887 & 108,832 \\
\bottomrule
\end{tabular}


==> tables/ibifsg_stats_thresh50.tex <==
\begin{tabular}{lllllll}
\toprule
Race & Accuracy & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
Asian & 0.989 & 0.913 & 0.878 & 0.895 & 0.758 & 9,244 \\
Black & 0.938 & 0.719 & 0.771 & 0.744 & 0.772 & 20,125 \\
Hispanic & 0.949 & 0.915 & 0.818 & 0.864 & 0.872 & 34,089 \\
White & 0.911 & 0.919 & 0.941 & 0.93 & 0.883 & 108,335 \\
\bottomrule
\end{tabular}


==> tables/ibisg_stats.tex <==
\begin{tabular}{lrrrrr}
\toprule
Race & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
asian & 0.859000 & 0.843000 & 0.851000 & 0.846000 & 12202 \\
black & 0.703000 & 0.655000 & 0.678000 & 0.905000 & 26059 \\
hispanic & 0.910000 & 0.806000 & 0.855000 & 0.924000 & 39089 \\
white & 0.875000 & 0.926000 & 0.900000 & 0.823000 & 122647 \\
\bottomrule
\end{tabular}


==> tables/ibisg_stats_max.tex <==
\begin{tabular}{lllllll}
\toprule
Race & Accuracy & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
Asian & 0.985 & 0.899 & 0.842 & 0.869 & 0.885 & 10,798 \\
Black & 0.915 & 0.69 & 0.676 & 0.683 & 0.951 & 24,777 \\
Hispanic & 0.943 & 0.91 & 0.794 & 0.848 & 0.951 & 37,176 \\
White & 0.882 & 0.882 & 0.929 & 0.905 & 0.908 & 111,314 \\
\bottomrule
\end{tabular}


==> tables/ibisg_stats_thresh50.tex <==
\begin{tabular}{lllllll}
\toprule
Race & Accuracy & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
Asian & 0.986 & 0.912 & 0.851 & 0.88 & 0.867 & 10,584 \\
Black & 0.919 & 0.698 & 0.684 & 0.691 & 0.917 & 23,896 \\
Hispanic & 0.945 & 0.915 & 0.802 & 0.855 & 0.937 & 36,636 \\
White & 0.887 & 0.887 & 0.933 & 0.909 & 0.9 & 110,406 \\
\bottomrule
\end{tabular}


==> tables/lookup_stats_max.tex <==
\begin{tabular}{lllllll}
\toprule
Race & Accuracy & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
Asian & 0.993 & 0.974 & 0.917 & 0.944 & 0.331 & 4,034 \\
Black & 0.933 & 0.683 & 0.629 & 0.655 & 0.231 & 6,029 \\
Hispanic & 0.955 & 0.936 & 0.891 & 0.913 & 0.4 & 15,622 \\
White & 0.904 & 0.898 & 0.937 & 0.917 & 0.274 & 33,593 \\
\bottomrule
\end{tabular}


==> tables/lookup_stats_thresh50.tex <==
\begin{tabular}{lllllll}
\toprule
Race & Accuracy & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
Asian & 0.993 & 0.974 & 0.918 & 0.946 & 0.329 & 4,020 \\
Black & 0.933 & 0.685 & 0.629 & 0.656 & 0.23 & 5,989 \\
Hispanic & 0.956 & 0.936 & 0.892 & 0.914 & 0.399 & 15,599 \\
White & 0.905 & 0.899 & 0.938 & 0.918 & 0.274 & 33,560 \\
\bottomrule
\end{tabular}


==> tables/ppp_bifsg_stats_thresh50.tex <==
\begin{tabular}{lllllll}
\toprule
Race & Accuracy & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
Asian & 0.991 & 0.952 & 0.838 & 0.891 & 0.562 & 6,854 \\
Black & 0.944 & 0.711 & 0.622 & 0.664 & 0.52 & 13,542 \\
Hispanic & 0.951 & 0.932 & 0.804 & 0.863 & 0.753 & 29,421 \\
White & 0.908 & 0.906 & 0.963 & 0.934 & 0.838 & 102,779 \\
\bottomrule
\end{tabular}


==> tables/ppp_bisg_stats_thresh50.tex <==
\begin{tabular}{lllllll}
\toprule
Race & Accuracy & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
Asian & 0.988 & 0.922 & 0.858 & 0.889 & 0.844 & 10,297 \\
Black & 0.922 & 0.703 & 0.688 & 0.695 & 0.892 & 23,239 \\
Hispanic & 0.946 & 0.919 & 0.806 & 0.859 & 0.926 & 36,214 \\
White & 0.89 & 0.889 & 0.936 & 0.912 & 0.887 & 108,805 \\
\bottomrule
\end{tabular}


==> tables/ppp_ensemble_stats_thresh50.tex <==
\begin{tabular}{lllllll}
\toprule
Race & Accuracy & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
Asian & 0.981 & 0.828 & 0.871 & 0.849 & 0.974 & 11,883 \\
Black & 0.935 & 0.716 & 0.821 & 0.765 & 0.971 & 25,298 \\
Hispanic & 0.946 & 0.9 & 0.811 & 0.853 & 0.983 & 38,442 \\
White & 0.905 & 0.925 & 0.921 & 0.923 & 0.987 & 121,105 \\
\bottomrule
\end{tabular}


==> tables/ppp_eth_stats_max.tex <==
\begin{tabular}{lllllll}
\toprule
Race & Accuracy & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
Asian & 0.974 & 0.897 & 0.643 & 0.749 & 1.0 & 12,202 \\
Black & 0.901 & 0.673 & 0.469 & 0.552 & 1.0 & 26,059 \\
Hispanic & 0.932 & 0.882 & 0.754 & 0.813 & 1.0 & 39,089 \\
White & 0.845 & 0.828 & 0.943 & 0.882 & 1.0 & 122,647 \\
\bottomrule
\end{tabular}


==> tables/ppp_eth_stats_thresh50.tex <==
\begin{tabular}{lllllll}
\toprule
Race & Accuracy & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
Asian & 0.977 & 0.918 & 0.667 & 0.773 & 0.919 & 11,214 \\
Black & 0.905 & 0.69 & 0.471 & 0.56 & 0.958 & 24,966 \\
Hispanic & 0.936 & 0.893 & 0.763 & 0.823 & 0.976 & 38,142 \\
White & 0.851 & 0.834 & 0.948 & 0.888 & 0.988 & 121,117 \\
\bottomrule
\end{tabular}


==> tables/ppp_fl_bayes_stats_thresh50.tex <==
\begin{tabular}{lllllll}
\toprule
Race & Accuracy & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
Asian & 0.976 & 0.766 & 0.871 & 0.816 & 0.979 & 11,947 \\
Black & 0.928 & 0.674 & 0.861 & 0.756 & 0.979 & 25,524 \\
Hispanic & 0.943 & 0.887 & 0.813 & 0.848 & 0.985 & 38,504 \\
White & 0.898 & 0.937 & 0.894 & 0.915 & 0.985 & 120,798 \\
\bottomrule
\end{tabular}


==> tables/ppp_fl_stats_thresh50.tex <==
\begin{tabular}{lllllll}
\toprule
Race & Accuracy & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
Asian & 0.977 & 0.788 & 0.851 & 0.818 & 0.977 & 11,925 \\
Black & 0.903 & 0.606 & 0.713 & 0.655 & 0.969 & 25,248 \\
Hispanic & 0.939 & 0.876 & 0.804 & 0.838 & 0.985 & 38,506 \\
White & 0.869 & 0.901 & 0.884 & 0.892 & 0.978 & 119,997 \\
\bottomrule
\end{tabular}


==> tables/ppp_ibifsg_stats_thresh50.tex <==
\begin{tabular}{lllllll}
\toprule
Race & Accuracy & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
Asian & 0.989 & 0.913 & 0.878 & 0.895 & 0.758 & 9,244 \\
Black & 0.938 & 0.719 & 0.771 & 0.744 & 0.772 & 20,125 \\
Hispanic & 0.949 & 0.915 & 0.818 & 0.864 & 0.872 & 34,089 \\
White & 0.911 & 0.919 & 0.941 & 0.93 & 0.883 & 108,335 \\
\bottomrule
\end{tabular}


==> tables/ppp_ibisg_stats_thresh50.tex <==
\begin{tabular}{lllllll}
\toprule
Race & Accuracy & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
Asian & 0.986 & 0.912 & 0.851 & 0.88 & 0.867 & 10,584 \\
Black & 0.919 & 0.698 & 0.684 & 0.691 & 0.917 & 23,896 \\
Hispanic & 0.945 & 0.915 & 0.802 & 0.855 & 0.937 & 36,636 \\
White & 0.887 & 0.887 & 0.933 & 0.909 & 0.9 & 110,406 \\
\bottomrule
\end{tabular}


==> tables/ppp_lookup_stats_max.tex <==
\begin{tabular}{lllllll}
\toprule
Race & Accuracy & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
Asian & 0.993 & 0.974 & 0.917 & 0.944 & 0.331 & 4,034 \\
Black & 0.933 & 0.683 & 0.629 & 0.655 & 0.231 & 6,029 \\
Hispanic & 0.955 & 0.936 & 0.891 & 0.913 & 0.4 & 15,622 \\
White & 0.904 & 0.898 & 0.937 & 0.917 & 0.274 & 33,593 \\
\bottomrule
\end{tabular}


==> tables/ppp_lookup_stats_thresh50.tex <==
\begin{tabular}{lllllll}
\toprule
Race & Accuracy & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
Asian & 0.993 & 0.974 & 0.918 & 0.946 & 0.329 & 4,020 \\
Black & 0.933 & 0.685 & 0.629 & 0.656 & 0.23 & 5,989 \\
Hispanic & 0.956 & 0.936 & 0.892 & 0.914 & 0.399 & 15,599 \\
White & 0.905 & 0.899 & 0.938 & 0.918 & 0.274 & 33,560 \\
\bottomrule
\end{tabular}


==> tables/ppp_rand_bifsg_stats_max.tex <==
\begin{tabular}{lllllll}
\toprule
Race & Accuracy & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
Asian & 0.991 & 0.934 & 0.827 & 0.877 & 0.597 & 5,100 \\
Black & 0.837 & 0.936 & 0.618 & 0.744 & 0.534 & 51,619 \\
Hispanic & 0.961 & 0.898 & 0.803 & 0.848 & 0.761 & 18,086 \\
White & 0.818 & 0.721 & 0.962 & 0.824 & 0.842 & 59,889 \\
\bottomrule
\end{tabular}


==> tables/ppp_rand_bifsg_stats_thresh50.tex <==
\begin{tabular}{lllllll}
\toprule
Race & Accuracy & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
Asian & 0.993 & 0.948 & 0.844 & 0.893 & 0.57 & 4,863 \\
Black & 0.842 & 0.938 & 0.624 & 0.749 & 0.518 & 50,045 \\
Hispanic & 0.963 & 0.906 & 0.808 & 0.854 & 0.751 & 17,851 \\
White & 0.822 & 0.729 & 0.964 & 0.83 & 0.837 & 59,531 \\
\bottomrule
\end{tabular}


==> tables/ppp_rand_bisg_stats_max.tex <==
\begin{tabular}{lllllll}
\toprule
Race & Accuracy & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
Asian & 0.989 & 0.873 & 0.846 & 0.859 & 0.878 & 7,501 \\
Black & 0.814 & 0.933 & 0.67 & 0.78 & 0.946 & 91,392 \\
Hispanic & 0.962 & 0.877 & 0.8 & 0.837 & 0.945 & 22,464 \\
White & 0.802 & 0.648 & 0.931 & 0.764 & 0.901 & 64,098 \\
\bottomrule
\end{tabular}


==> tables/ppp_rand_bisg_stats_thresh50.tex <==
\begin{tabular}{lllllll}
\toprule
Race & Accuracy & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
Asian & 0.991 & 0.9 & 0.863 & 0.881 & 0.847 & 7,232 \\
Black & 0.825 & 0.937 & 0.683 & 0.79 & 0.888 & 85,801 \\
Hispanic & 0.964 & 0.889 & 0.812 & 0.849 & 0.925 & 21,974 \\
White & 0.813 & 0.668 & 0.937 & 0.78 & 0.886 & 63,013 \\
\bottomrule
\end{tabular}


==> tables/ppp_rand_ensemble_stats_max.tex <==
\begin{tabular}{lllllll}
\toprule
Race & Accuracy & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
Asian & 0.983 & 0.767 & 0.867 & 0.814 & 1.0 & 8,539 \\
Black & 0.884 & 0.939 & 0.812 & 0.871 & 1.0 & 96,589 \\
Hispanic & 0.961 & 0.856 & 0.807 & 0.831 & 1.0 & 23,763 \\
White & 0.874 & 0.772 & 0.916 & 0.838 & 1.0 & 71,109 \\
\bottomrule
\end{tabular}


==> tables/ppp_rand_ensemble_stats_thresh50.tex <==
\begin{tabular}{lllllll}
\toprule
Race & Accuracy & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
Asian & 0.985 & 0.801 & 0.876 & 0.837 & 0.974 & 8,313 \\
Black & 0.89 & 0.941 & 0.822 & 0.878 & 0.97 & 93,686 \\
Hispanic & 0.963 & 0.867 & 0.816 & 0.841 & 0.984 & 23,373 \\
White & 0.88 & 0.783 & 0.922 & 0.847 & 0.987 & 70,201 \\
\bottomrule
\end{tabular}


==> tables/ppp_rand_eth_stats_max.tex <==
\begin{tabular}{lllllll}
\toprule
Race & Accuracy & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
Asian & 0.979 & 0.837 & 0.64 & 0.725 & 1.0 & 8,539 \\
Black & 0.725 & 0.927 & 0.468 & 0.622 & 1.0 & 96,589 \\
Hispanic & 0.952 & 0.826 & 0.758 & 0.79 & 1.0 & 23,763 \\
White & 0.701 & 0.546 & 0.943 & 0.691 & 1.0 & 71,109 \\
\bottomrule
\end{tabular}


==> tables/ppp_rand_eth_stats_thresh50.tex <==
\begin{tabular}{lllllll}
\toprule
Race & Accuracy & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
Asian & 0.982 & 0.867 & 0.664 & 0.752 & 0.92 & 7,856 \\
Black & 0.731 & 0.933 & 0.471 & 0.626 & 0.96 & 92,763 \\
Hispanic & 0.956 & 0.847 & 0.767 & 0.805 & 0.976 & 23,201 \\
White & 0.705 & 0.554 & 0.948 & 0.7 & 0.988 & 70,246 \\
\bottomrule
\end{tabular}


==> tables/ppp_rand_fl_bayes_stats_max.tex <==
\begin{tabular}{lllllll}
\toprule
Race & Accuracy & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
Asian & 0.979 & 0.708 & 0.869 & 0.78 & 0.994 & 8,490 \\
Black & 0.897 & 0.926 & 0.855 & 0.889 & 1.0 & 96,547 \\
Hispanic & 0.959 & 0.841 & 0.811 & 0.826 & 0.999 & 23,734 \\
White & 0.889 & 0.816 & 0.889 & 0.851 & 1.0 & 71,075 \\
\bottomrule
\end{tabular}


==> tables/ppp_rand_fl_bayes_stats_thresh50.tex <==
\begin{tabular}{lllllll}
\toprule
Race & Accuracy & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
Asian & 0.981 & 0.732 & 0.876 & 0.798 & 0.981 & 8,379 \\
Black & 0.903 & 0.929 & 0.863 & 0.895 & 0.979 & 94,523 \\
Hispanic & 0.961 & 0.848 & 0.818 & 0.833 & 0.986 & 23,426 \\
White & 0.895 & 0.825 & 0.895 & 0.859 & 0.985 & 70,067 \\
\bottomrule
\end{tabular}


==> tables/ppp_rand_fl_stats_max.tex <==
\begin{tabular}{lllllll}
\toprule
Race & Accuracy & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
Asian & 0.979 & 0.723 & 0.841 & 0.777 & 1.0 & 8,539 \\
Black & 0.819 & 0.9 & 0.703 & 0.789 & 1.0 & 96,589 \\
Hispanic & 0.956 & 0.82 & 0.802 & 0.811 & 1.0 & 23,763 \\
White & 0.811 & 0.682 & 0.876 & 0.767 & 1.0 & 71,109 \\
\bottomrule
\end{tabular}


==> tables/ppp_rand_fl_stats_thresh50.tex <==
\begin{tabular}{lllllll}
\toprule
Race & Accuracy & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
Asian & 0.981 & 0.739 & 0.852 & 0.792 & 0.979 & 8,357 \\
Black & 0.825 & 0.906 & 0.71 & 0.796 & 0.969 & 93,607 \\
Hispanic & 0.957 & 0.827 & 0.809 & 0.818 & 0.987 & 23,448 \\
White & 0.817 & 0.69 & 0.884 & 0.775 & 0.978 & 69,545 \\
\bottomrule
\end{tabular}


==> tables/ppp_rand_ibifsg_stats_max.tex <==
\begin{tabular}{lllllll}
\toprule
Race & Accuracy & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
Asian & 0.991 & 0.889 & 0.877 & 0.883 & 0.77 & 6,573 \\
Black & 0.871 & 0.94 & 0.768 & 0.845 & 0.786 & 75,939 \\
Hispanic & 0.963 & 0.878 & 0.817 & 0.846 & 0.877 & 20,850 \\
White & 0.861 & 0.755 & 0.939 & 0.837 & 0.888 & 63,133 \\
\bottomrule
\end{tabular}


==> tables/ppp_rand_ibifsg_stats_thresh50.tex <==
\begin{tabular}{lllllll}
\toprule
Race & Accuracy & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
Asian & 0.991 & 0.9 & 0.883 & 0.891 & 0.763 & 6,512 \\
Black & 0.875 & 0.941 & 0.773 & 0.849 & 0.774 & 74,723 \\
Hispanic & 0.964 & 0.884 & 0.821 & 0.852 & 0.87 & 20,665 \\
White & 0.864 & 0.76 & 0.941 & 0.841 & 0.884 & 62,858 \\
\bottomrule
\end{tabular}


==> tables/ppp_rand_ibisg_stats_max.tex <==
\begin{tabular}{lllllll}
\toprule
Race & Accuracy & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
Asian & 0.989 & 0.87 & 0.847 & 0.858 & 0.889 & 7,587 \\
Black & 0.814 & 0.933 & 0.671 & 0.781 & 0.95 & 91,728 \\
Hispanic & 0.962 & 0.875 & 0.8 & 0.836 & 0.95 & 22,581 \\
White & 0.802 & 0.649 & 0.93 & 0.765 & 0.907 & 64,498 \\
\bottomrule
\end{tabular}


==> tables/ppp_rand_ibisg_stats_thresh50.tex <==
\begin{tabular}{lllllll}
\toprule
Race & Accuracy & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
Asian & 0.99 & 0.889 & 0.856 & 0.872 & 0.87 & 7,428 \\
Black & 0.821 & 0.936 & 0.679 & 0.787 & 0.914 & 88,314 \\
Hispanic & 0.964 & 0.885 & 0.808 & 0.845 & 0.936 & 22,235 \\
White & 0.808 & 0.661 & 0.934 & 0.774 & 0.9 & 63,974 \\
\bottomrule
\end{tabular}


==> tables/ppp_rand_lookup_stats_max.tex <==
\begin{tabular}{lllllll}
\toprule
Race & Accuracy & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
Asian & 0.995 & 0.971 & 0.923 & 0.946 & 0.326 & 2,787 \\
Black & 0.83 & 0.931 & 0.636 & 0.755 & 0.232 & 22,368 \\
Hispanic & 0.968 & 0.921 & 0.892 & 0.907 & 0.399 & 9,475 \\
White & 0.816 & 0.675 & 0.938 & 0.785 & 0.272 & 19,372 \\
\bottomrule
\end{tabular}


==> tables/ppp_rand_lookup_stats_thresh50.tex <==
\begin{tabular}{lllllll}
\toprule
Race & Accuracy & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
Asian & 0.995 & 0.974 & 0.925 & 0.949 & 0.325 & 2,776 \\
Black & 0.831 & 0.932 & 0.637 & 0.757 & 0.23 & 22,232 \\
Hispanic & 0.968 & 0.922 & 0.893 & 0.907 & 0.398 & 9,467 \\
White & 0.817 & 0.677 & 0.939 & 0.787 & 0.272 & 19,353 \\
\bottomrule
\end{tabular}


==> tables/ppp_rand_reth_stats_max.tex <==
\begin{tabular}{lllllll}
\toprule
Race & Accuracy & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
Asian & 0.942 & 0.417 & 0.882 & 0.567 & 1.0 & 8,539 \\
Black & 0.793 & 0.799 & 0.762 & 0.78 & 1.0 & 96,589 \\
Hispanic & 0.948 & 0.792 & 0.767 & 0.779 & 1.0 & 23,763 \\
White & 0.796 & 0.727 & 0.683 & 0.704 & 1.0 & 71,109 \\
\bottomrule
\end{tabular}


==> tables/ppp_rand_reth_stats_thresh50.tex <==
\begin{tabular}{lllllll}
\toprule
Race & Accuracy & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
Asian & 0.95 & 0.475 & 0.905 & 0.623 & 0.958 & 8,179 \\
Black & 0.818 & 0.822 & 0.798 & 0.81 & 0.893 & 86,272 \\
Hispanic & 0.956 & 0.834 & 0.801 & 0.817 & 0.928 & 22,057 \\
White & 0.822 & 0.759 & 0.71 & 0.734 & 0.864 & 61,430 \\
\bottomrule
\end{tabular}


==> tables/ppp_reth_stats_max.tex <==
\begin{tabular}{lllllll}
\toprule
Race & Accuracy & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
Asian & 0.939 & 0.502 & 0.882 & 0.64 & 1.0 & 12,202 \\
Black & 0.811 & 0.386 & 0.763 & 0.513 & 1.0 & 26,059 \\
Hispanic & 0.926 & 0.845 & 0.761 & 0.801 & 1.0 & 39,089 \\
White & 0.763 & 0.909 & 0.682 & 0.779 & 1.0 & 122,647 \\
\bottomrule
\end{tabular}


==> tables/ppp_reth_stats_thresh50.tex <==
\begin{tabular}{lllllll}
\toprule
Race & Accuracy & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
Asian & 0.947 & 0.563 & 0.902 & 0.693 & 0.961 & 11,724 \\
Black & 0.829 & 0.42 & 0.798 & 0.551 & 0.892 & 23,250 \\
Hispanic & 0.935 & 0.879 & 0.793 & 0.834 & 0.929 & 36,326 \\
White & 0.79 & 0.922 & 0.709 & 0.802 & 0.864 & 105,936 \\
\bottomrule
\end{tabular}


==> tables/reth_stats.tex <==
\begin{tabular}{lrrrrr}
\toprule
Race & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
asian & 0.466000 & 0.870000 & 0.607000 & 1.000000 & 12202 \\
black & 0.385000 & 0.743000 & 0.507000 & 1.000000 & 26059 \\
hispanic & 0.830000 & 0.763000 & 0.795000 & 1.000000 & 39089 \\
white & 0.907000 & 0.673000 & 0.773000 & 1.000000 & 122647 \\
\bottomrule
\end{tabular}


==> tables/reth_stats_thresh50.tex <==
\begin{tabular}{lllllll}
\toprule
Race & Accuracy & Precision & Recall & F1 Score & Coverage & Support \\
\midrule
Asian & 0.947 & 0.563 & 0.902 & 0.693 & 0.961 & 11,724 \\
Black & 0.829 & 0.42 & 0.798 & 0.551 & 0.892 & 23,250 \\
Hispanic & 0.935 & 0.879 & 0.793 & 0.834 & 0.929 & 36,326 \\
White & 0.79 & 0.922 & 0.709 & 0.802 & 0.864 & 105,936 \\
\bottomrule
\end{tabular}

